TranSplat: Generalizable 3D Gaussian Splatting from Sparse Multi-View Images with Transformers

Compared with previous 3D reconstruction methods like Nerf, recent Generalizable 3D Gaussian Splatting (G-3DGS) methods demonstrate impressive efficiency even in the sparse-view setting. However, the promising reconstruction performance of existing G-3DGS methods relies heavily on accurate multi-view feature matching, which is quite challenging. Especially for the scenes that have many non-overlapping areas between various views and contain numerous similar regions, the matching performance of existing methods is poor and the reconstruction precision is limited. To address this problem, we develop a strategy that utilizes a predicted depth confidence map to guide accurate local feature matching. In addition, we propose to utilize the knowledge of existing monocular depth estimation models as prior to boost the depth estimation precision in non-overlapping areas between views. Combining the proposed strategies, we present a novel G-3DGS method named TranSplat, which obtains the best performance on both the RealEstate10K and ACID benchmarks while maintaining competitive speed and presenting strong cross-dataset generalization ability. Our code, and demos will be available at: https://xingyoujun.github.io/transplat.

==> sections/checklist.tex <==
\section*{CheckList}
This paper:

Includes a conceptual outline and/or pseudocode description of AI methods introduced (\underline{}{yes}/partial/no/NA)

Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (\underline{yes}/no)

Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (\underline{yes}/no)

Does this paper make theoretical contributions? (yes/\underline{no})

Does this paper rely on one or more datasets? (\underline{yes}/no)

A motivation is given for why the experiments are conducted on the selected datasets (\underline{yes}/partial/no/NA)

All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/\underline{NA})

All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/\underline{NA})

All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (\underline{yes}/no/NA)

All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (\underline{yes}/partial/no/\underline{NA})

All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/\underline{NA})

Does this paper include computational experiments? (\underline{yes}/no)

Any code required for pre-processing data is included in the appendix. (\underline{yes}/partial/no).

All source code required for conducting and analyzing the experiments is included in a code appendix. (\underline{yes}/partial/no)

All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\underline{yes}/partial/no)

All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (\underline{yes}/partial/no)

If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/\underline{NA})

This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/\underline{partial}/no)

This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (\underline{yes}/partial/no)

This paper states the number of algorithm runs used to compute each reported result. (\underline{yes}/no)

Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (\underline{yes}/no)

The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/\underline{no})

This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (\underline{yes}/partial/no/NA)

This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/\underline{partial}/no/NA)
